Secret Sharing Sharing For Highly Scalable Secure Aggregation

Secure Multiparty Computation (MPC) can improve the security and privacy of data owners while allowing analysts to perform high quality analytics. Secure aggregation is a secure distributed mechanism to support federated deep learning without the need for trusted third parties. In this paper we present a highly performant secure aggregation protocol with sub-linear communication complexity. Our protocol achieves greater communication and computation efficiencies through a group-based approach. It is similar to secret sharing protocols extended to vectors of values-aka gradients-but within groups we add an additional layer of secret sharing of shares themselves-aka sharding. This ensures privacy of secret inputs in the standard real/ideal security paradigm, in both semi-honest and malicious settings where the server may collude with the adversary. In the malicious setting with 5% corrupt clients and 5% dropouts, our protocol can aggregate over a federation with 100,000,000 members and vectors of length 100 while requiring each client to communicate with only 350 other clients. The concrete computation cost for this aggregation is less than half a second for the server and less than 100ms for the client.

==> ces-macros.tex <==
\RequirePackage{ifthen}

\renewcommand{\TirName}[1]{\textsc{#1}}

% !!! removed to build OOPSLA
% \renewcommand{\thetheorem}{\thesection.\arabic{theorem}}
% \renewcommand{\thelemma}{\thesection.\arabic{lemma}}
% \renewcommand{\theexample}{\thesection.\arabic{example}}
% \renewcommand{\thedefinition}{\thesection.\arabic{definition}}
% \renewcommand{\theproposition}{\thesection.\arabic{proposition}}
% \renewcommand{\thecorollary}{\thesection.\arabic{corollary}}

% !!! removed to build OOPSLA
% \numberwithin{theorem}{section}
% \numberwithin{lemma}{section}
% \numberwithin{example}{section}
% \numberwithin{definition}{section}
% \numberwithin{proposition}{section}
% \numberwithin{corollary}{section}

% !!! removed to build APLAS
% \ifthenelse{\equal{\theoremdefns}{0}}
% {
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{example}[theorem]{Example}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{proposition}[theorem]{Proposition}
% \newenvironment{proof}{\noindent\textit{Proof. }}{}
% % \newcommand{\qed}{$\Box$}
% \def\squareforqed{\hbox{\rlap{$\sqcap$}$\sqcup$}}
% \def\qed{\ifmmode\squareforqed\else{\unskip\nobreak\hfil
% \penalty50\hskip1em\null\nobreak\hfil\squareforqed
% \parfillskip=0pt\finalhyphendemerits=0\endgraf}\fi}
% }
% {}

% \ifthenelse{\equal{\theoremdefns}{1}}
% {
% \newtheorem{theorem}{Theorem}
% \newtheorem{definition}{Definition}
% \newtheorem{corollary}{Corollary}
% \newtheorem{example}{Example}
% \newtheorem{lemma}{Lemma}
% \newtheorem{proposition}{Proposition}
% \def\squareforqed{\hbox{\rlap{$\sqcap$}$\sqcup$}}
% \def\qed{\ifmmode\squareforqed\else{\unskip\nobreak\hfil
% \penalty50\hskip1em\null\nobreak\hfil\squareforqed
% \parfillskip=0pt\finalhyphendemerits=0\endgraf}\fi}
% }
% {}

\newcommand{\cesnote}[1]{\textit{(#1 -- c.e.s.)}}
\newcommand{\snote}[1]{{\small \textbf{\textit{(#1 -- Scott)}}}}
\newcommand{\dcdnote}[1]{{\color{magenta}\it (#1 -- {d.c.d.})}}

%\def\longhtobpa#1{\text{BPA}(#1)}
%\def\shorthtobpa#1{#1} % ignore BPA translation in short version

%\long\def\eatit#1{}
%\long\def\spititback#1{#1}
%\long\def\spitsmaller#1{{\def\formulasize{\scriptsize} {\scriptsize #1}}}
%\def\shortversion{\def\condensed{\spititback} \def\cut{\eatit}\def\htobpa{\shorthtobpa}}
%\def\longversion{\def\condensed{\eatit} \def\cut{\spititback}\def\htobpa{\longhtobpa}}
%\def\shortversionshowlongs{\def\condensed{\spititback} \def\cut{\spitsmaller}}
%\shortversion


\newcommand{\colfigurebox}[5]
{
        \begin{figure}
        \begin{center}
        \framebox[#1]{
                \begin{minipage}{#2}
                \footnotesize
                \vspace{2mm}
                #5
                \vspace{1mm}
                \end{minipage}
                \normalsize
        }
        \caption{#4} 
        \label{#3}
        \end{center}
        \end{figure}
}

\newcommand{\figurebox}[5]
{
        \begin{figure*}
        \begin{center}
        \framebox[#1]{
                \begin{minipage}{#2}
                \footnotesize
                \vspace{2mm}
                #5
                \vspace{1mm}
                \end{minipage}
                \normalsize
        }
        \caption{#4} 
        \label{#3}
        \end{center}
        \end{figure*}
}

%%%%% dduct %%%%%%
\newcommand{\dduct}[2]{
\ensuremath{
\renewcommand{\arraystretch}{1.3}
        \begin{array}[b]{c}
                #1\\\hline
                #2
        \end{array}
\renewcommand{\arraystretch}{1}
}
}
%%%%%%%%%%%%%%%%%%%

\newcommand{\algtab}[1]
{
\vspace*{-3mm}
\begin{tabbing}
\hspace*{12mm}\=\hspace{9mm}\=\hspace{9mm}\=\hspace{6mm}\=\hspace{6mm}\=
\hspace{6mm}\=\\\newcommand{\cmnts}{\noindent\textbf{Comments\hspace{2mm}}}
#1
\end{tabbing}
}
\newcommand{\lt}{\left\{}
\newcommand{\rt}{\right\}}
\newcommand{\Lt}{\left\{\!\!\right.}
\newcommand{\Rt}{\left.\!\!\right\}}
\newcommand{\const}{\mathbf{c}}
\newcommand{\heading}[1]{\noindent\textbf{#1\ \  }}

\newcommand{\schemecomp}[3]{#1\vdash^i#2\preccurlyeq#3}

\newcommand{\Estep}{\rightarrow}
\newcommand{\instance}{\preccurlyeq}
\newcommand{\geninstance}{\trianglelefteq}
\newcommand{\gen}{\mathit{gen}}
\newcommand{\genvars}{\mathit{genvars}}

\newcommand{\iruleone}{\textsc{Sub$^\instance$}}
\newcommand{\iruletwo}{$(\preccurlyeq\!\forall)$}
\newcommand{\irulethree}{$(\forall\!\preccurlyeq)$}

%\newcommand{\seclang}{\lambda_{\text{\rm sec}}}
%\newcommand{\setlang}{\lambda_{\text{\rm set}}}
\newcommand{\pinit}{\ensuremath{p_0}}
\newcommand{\reduce}{\leadsto}
\newcommand{\ctxreduce}{\rightarrow}
%\newcommand{\eqdefn}{=_{\scriptscriptstyle{\mathit{def}}}}
\newcommand{\subn}{\psi}
\newcommand{\subndefn}[1]{[#1]}
\newcommand{\restrict}[2]{{#1}\!\mid_{#2}}
\newcommand{\rrow}[2]{\lt \drow{r}{#1}{#2} \rt}
\newcommand{\refcell}{\mathrm{ref}}
\newcommand{\tref}{\mathrm{ref}}
\newcommand{\hmxconfig}[2]{#1/#2}
%\newcommand{\store}{\varsigma}
\newcommand{\rangevec}[3]{#1^{\hspace{4pt}#2 \in \setdefn{1,\ldots,#3}}}
\newcommand{\initenv}{\Delta}
\newcommand{\extend}[3]{#1[#2 \mapsto #3]}
\newcommand{\gdesc}[1]{\text{\textit{#1}}}
%\newcommand{\loc}{l}
\newcommand{\setdefn}[1]{\lt#1\rt}
\newcommand{\deref}{\,!}
\newcommand{\assignfn}[1]{{:=}_{#1}}
%\renewcommand{\eabs}[3]{\lambda\langle#1\rangle #2 . #3 }
\newcommand{\credentials}{\mathcal{A}}
\newcommand{\constrain}[2]{#1\!\mid_{#2}}
\newcommand{\subrule}{\TirName{Sub}}
\newcommand{\varrule}{\TirName{Var}}
\newcommand{\locrule}{\TirName{Loc}}
\newcommand{\absrule}{\TirName{Abs}}
\newcommand{\apprule}{\TirName{App}}
\newcommand{\letrule}{\TirName{Let}}
\newcommand{\assignrule}{\TirName{Assign}}
\newcommand{\construle}{\TirName{Const}}
\newcommand{\refrule}{\TirName{Ref}}
\newcommand{\derefrule}{\TirName{Deref}}
\newcommand{\forallelim}{\TirName{$\forall$ Elim}}
\newcommand{\forallintro}{\TirName{$\forall$ Intro}}
\newcommand{\configrule}{\TirName{Config}}
\newcommand{\allv}{\beta}
\newcommand{\svar}{\alpha}
\newcommand{\vvec}{\bar{\allv}}
\newcommand{\tvec}{\bar{\tau}}
\newcommand{\existsC}[2]{\exists #1 . #2}
\newcommand{\rename}{\varrho}
\newcommand{\metaj}{\mathcal{J}}
\newcommand{\eass}[1]{\mathord{:=}\,#1}
\newcommand{\eassign}[2]{\mathord{:=}\,#1\,#2}
\newcommand{\cesqed}{}
\newcommand{\sys}{\ensuremath{\system{1}{=}}}
\newcommand{\etal}{\emph{et al.}}
%\newcommand{\enabler}{\mathrm{enable}_r}
%\newcommand{\requirer}{\mathrm{require}_r}
\newcommand{\defeq}{\triangleq}
\newcommand{\bestAttc}{\text{\it tryKill'}}
\newcommand{\labs}[2]{\lambda #1 . #2}
\newcommand{\menabler}{\ensuremath{{\text{\it maybeEnable}}_r}}
\newcommand{\action}{\text{\it action}}
\newcommand{\tin}{\tpre}
\newcommand{\tout}{\tabs}
\newcommand{\allsett}{\urow{\tin}}
\newcommand{\nonesett}{\urow{\tout}}
\newcommand{\snext}{\tnext}
%\newcommand{\fielduk}[2]{\stackrel{\;#2}{#1}}
\newcommand{\fielduk}[2]{#1:#2}
\newcommand{\fieldint}[1]{\fielduk{#1}{\tin}}
\newcommand{\fieldoutt}[1]{\fielduk{#1}{\tout}}
%\newcommand{\fieldint}[1]{\dot{#1}}
%\newcommand{\fieldoutt}[1]{\bar{#1}}
\newcommand{\srow}[3]{\fielduk{#1}{#2}\snext#3}
\newcommand{\trule}[1]{\textsc{#1}}
\newcommand{\etrue}{\fpkeyword{true}}
\newcommand{\efalse}{\fpkeyword{false}}
\newcommand{\boolt}{\textit{bool}}
\newcommand{\unitt}{\textit{unit}}
\newcommand{\unroll}[2]{\circlearrowright_{#1}#2}
\newcommand{\acclang}{\ensuremath{\lambda_{\mathrm{trace}}}}
\newcommand{\histlang}{\acclang}
%\newcommand{\stacklang}{\ensuremath{\lambda_{\mathrm{trace}}}}
\newcommand{\stacklang}{\ensuremath{\acclang^{\hstack}}}
\newcommand{\hist}{\theta}
\newcommand{\hconfig}[2]{#1,#2}
\newcommand{\hlog}[2]{#1;#2}
\newcommand{\boolinterp}[1]{\cod{#1}_\mathrm{bool}}
\newcommand{\squeeze}[1]{\hat{#1}}
\newcommand{\bigsqueeze}[1]{\widehat{#1}}
\newcommand{\scontextfn}{\text{context}}
\newcommand{\scontext}[2]{\scontextfn_{#1}(#2)}
\newcommand{\slength}{\text{length}}
\newcommand{\fdepth}{\text{fdepth}}
\newcommand{\sframefn}{\text{frame}}
\newcommand{\sframe}[2]{\sframefn_{#1}(#2)}
\newcommand{\hjudge}[4]{#1, #2 \vdash #3 : #4}
\newcommand{\hcijudge}[5]{#1, #2 \vdash_{#3} #4 : #5}
\newcommand{\hijudge}[4]{#1, #2 \vdash_{W} #3 : #4}
\newcommand{\hcjudge}[5]{#1, #2, #3 \vdash #4 : #5}
\newcommand{\lhjudge}[5]{#1, #2, #3 \vdash #4 : #5}
\newcommand{\gchjudge}[5]{#1, #2, #3 \vdash #4 : #5}
\newcommand{\labinferrule}[3]{\inferrule*[right=\scriptsize#3]{#1}{#2}}
\newcommand{\linfer}[3]{\inferrule*[right=\textsc{\scriptsize#3}]{#1}{#2}}
\newcommand{\Labinferrule}[3]{\inferrule*[Right=\scriptsize#3]{#1}{#2}}
\newcommand{\singleton}[1]{\tset{#1}}
\newcommand{\tsetp}[1]{\tset{\cdot#1\cdot}}
\newcommand{\arrowt}[1]{\xrightarrow{#1}}
\newcommand{\arrowht}[3]{#1 \arrowt{#2} #3}
\newcommand{\HC}{\mathit{HC}}
\newcommand{\evsig}{\Sigma}
\newcommand{\logbook}{\varsigma}
\newcommand{\logbookt}{\Sigma}
\newcommand{\hid}{\iota}
\newcommand{\hdecl}[2]{\fpkeyword{history }#1\text{ in }#2}
\newcommand{\lev}[1]{\ev_{#1}}
\newcommand{\lcheck}[2]{#1_{#2}}
\newcommand{\hsubn}{\psi}
\newcommand{\evpush}{\mathrm{push}}
\newcommand{\evpop}{\mathrm{pop}}
\newcommand{\stackify}{\mathit{stackify}}
\newcommand{\inspect}{\mathit{inspect}}
\newcommand{\fresh}[1]{#1 \text{ fresh}}
\newcommand{\pdistinct}[1]{#1 \text{ p-distinct}}
%\newcommand{\enew}[2]{\fpkeyword{new}\ #1\ \fpkeyword{in}\ #2}
\newcommand{\enew}[2]{\fpkeyword{new}\ #1\ \fpkeyword{in}\ #2}
\newcommand{\sexists}[2]{\exists #1 . \singleton{#2}}
\newcommand{\gcvar}{\zeta}
\newcommand{\gcvvec}{\bar\zeta}
\newcommand{\gcarrowt}[4]{\nabla #1 . #2 \xrightarrow{#3} #4}
\newcommand{\variantt}[1]{[#1]}
%\newcommand{\kind}[2]{#1:#2}
\newcommand{\ksingle}{\textit{Sing}}
\newcommand{\khistory}{\textit{Eff}}
%\newcommand{\kgcsingle}{\text{\emph{Single}}_{\gcvar}}
\newcommand{\ktype}{\textit{Type}}
\newcommand{\fvgc}[1]{\text{\rm fv}_\gcvar(#1)}
%\newcommand{\tvset}[1]{\mathcal{V}_{#1}}
\newcommand{\hvvec}{\bar{h}}
\newcommand{\cvec}{\bar{c}}
\newcommand{\gchist}[2]{\nabla #1 . #2}
\newcommand{\truncate}[1]{#1\backslash_{\mu}}
\newcommand{\trace}{\vartheta}
\newcommand{\Trace}{\Theta}
\newcommand{\halt}{\fpkeyword{halt}}
\newcommand{\diverge}{\uparrow}
\newcommand{\aftrans}[1]{\stackrel{#1}{\leadsto}}
\newcommand{\intersect}{\mathit{intersect}}
\newcommand{\demand}{\mathit{demand}}
\newcommand{\hfloor}[1]{\lfloor #1 \rfloor}
\newcommand{\ncod}[2]{\lfloor #2 \rfloor_{#1}}
\newcommand{\hbasis}{\mathit{basis}}
\newcommand{\hbases}{\mathit{bases}}
\newcommand{\metalet}[3]{\text{let}\,#1=#2\,\text{in}\,#3}
\newcommand{\metaite}[3]{\text{if}\,#1\,\text{then}\,#2\,\text{else}\,#3}
\newcommand{\ltrans}[1]{\xrightarrow{#1}}
\newcommand{\gcltrans}[2]{\xrightarrow{#2}_{#1}}
%\newcommand{\acclangver}[1]{\lambda_{\mathrm{trace}}^{#1}}
\newcommand{\bpatrans}[2]{{\text{BPA}(#1,#2) }}
%\newcommand{\evkeyword}[1]{\scriptstyle{\mathbf{#1}}}
\newcommand{\evkeyword}[1]{{\mathrm{#1}}}
\newcommand{\evenable}[1]{\mathrm{enable}_#1}
\newcommand{\phiinsp}{\phi_\text{inspect}}
\newcommand{\phiinspect}[1]{\phi_{\text{inspect,}#1}}
\newcommand{\phienable}[1]{\phi_{\text{enable,}#1}}
\newcommand{\phiamplify}[1]{\phi_{\text{amplify,}#1}}
\newcommand{\evinspect}[1]{\phiinspect{#1}}
\newcommand{\evamplify}[1]{\fpkeyword{amplify}_{#1}}
\newcommand{\evdemand}[1]{\fpkeyword{demand}_{#1}}
\newcommand{\evmgr}{\fpkeyword{mgr}}
\newcommand{\evacct}{\fpkeyword{acct}}
\newcommand{\evcrit}{\fpkeyword{crit}}
%\newcommand{\trans}[1]{\langle #1 \rangle}
\newcommand{\trans}[1]{( #1 )}
%\newcommand{\alltrans}[1]{[ #1 ]}
\newcommand{\nowlab}{\mathrm{Now}}
\newcommand{\pc}[1]{#1\!\!\downarrow}
\newcommand{\cvar}{\chi}
\newcommand{\existsend}{\trans{\mathrm{Now}}}
%\newcommand{\allend}{[ \mathrm{Now} ]}
\newcommand{\evdelim}{\circ}
\newcommand{\evldelim}{\rhd}
\newcommand{\evrdelim}{\lhd}
\newcommand{\muenable}[1]{\phi_{\text{enable-ok,#1}}}
\newcommand{\muinspect}[1]{\phi_{\text{inspect-ok,#1}}}
\newcommand{\muamplify}{\text{amplify}}
\newcommand{\mudemand}{\text{demand}}
\newcommand{\phidemand}[1]{\phi_{\text{demand},#1}}
\newcommand{\phidemandone}[1]{\phi_{\text{demand1},#1}}
\newcommand{\phidemandtwo}[1]{\phi_{\text{demand2},#1}}
\newcommand{\jsicheck}{\text{checkit}}
\newcommand{\jsienable}{\text{enableit}}
\newcommand{\filewpriv}{{r{:}\evkeyword{filew}}}
\newcommand{\htoX}{\Psi}
\newcommand{\mumu}{\mbox{\boldmath{$\mu$}}}
\newcommand{\munu}{\mbox{\boldmath{$\nu$}}}
\newcommand{\pinterp}{\Pi}
\newcommand{\staticpinterp}{\Pi_{\mu}}
\newcommand{\muinterp}[2]{\llbracket#1\rrbracket^{#2}}
\newcommand{\preprocess}{\text{pp}}
\newcommand{\emptystack}{\text{nil}}
\newcommand{\dotstack}{\varsigma}
\newcommand{\hframe}{\mathit{frame}}
\newcommand{\systemp}{{p{:}\evkeyword{system}}}
\newcommand{\acctp}{{p{:}\evkeyword{acct}}}
\newcommand{\Poccurs}[1]{\text{occurs}(#1)}
\newcommand{\jgmt}{\mathcal{J}}
\newcommand{\erase}{\text{erase}_\hist}
\newcommand{\terase}{\text{erase}_H}
\newcommand{\stjudge}[3]{#1 \vdash #2 : #3}
\newcommand{\ltsV}{V}
\newcommand{\muentails}[1]{\Vdash_{#1}}
\renewcommand{\implies}{\Rightarrow}
\newcommand{\simplecheck}{\phi}
\newcommand{\contains}{\sqsupseteq}
\newcommand{\stacked}[1]{{\cdot{#1}\cdot}}
\newcommand{\cons}[2]{\ensuremath{#1\!::\!#2}}
\newcommand{\hstack}{\ensuremath{\mathtt{S}}}
\newcommand{\hists}{\mathcal{H}}
\newcommand{\flowsto}{\sqsubseteq}
\newcommand{\closure}{\mathit{close}}
\newcommand{\hclosure}{\mathit{hclose}}
\newcommand{\mgu}{\mathit{MGS}}
\newcommand{\unifysoln}{\mathit{soln}}
\renewcommand{\scheme}[3]{\forall#1.#3/#2}
\newcommand{\po}{\preccurlyeq}
\newcommand{\hlt}{\preccurlyeq}
\newcommand{\monot}{\hat{\tau}}
\newcommand{\interp}{\rho}
\newcommand{\unify}{\mathit{unify}}
\newcommand{\subtype}[2]{#1\, \flowsto\, #2}
\newcommand{\hextract}{\mathit{hextract}}
\newcommand{\hextractC}{\mathit{hextract}_{C}}
\newcommand{\sextract}{\mathit{sextract}}
\newcommand{\ctrans}{\leadsto_\mathit{close}}
\newcommand{\ctransctx}{\rightarrow_\mathit{close}}
\newcommand{\close}{\mathit{close}}
\newcommand{\hclose}{\mathit{hclose}}
\newcommand{\bounds}{\mathit{bounds}}
\newcommand{\hsplit}{\mathit{hsplit}}
\newcommand{\cok}[1]{\vdash #1 : \mathit{ok}}
\newcommand{\habstract}[2]{\mathit{abstract}(#1,#2)}
\newcommand{\HX}{\mathit{HX}}
\newcommand{\mut}[2]{\mu #1 . #2}

\def\with{\ \mathit{with}\ }
\def\requiring{\ \mathit{requiring}\ }
\def\nothing{\mathit{nada}}
\def\ev{\mathit{e\!v}}
\def\Ev{\mathit{E\!\!V}}
\def\check{\fpkeyword{check}\ }
\def\unit{\fpkeyword{unit}}
\def\emptyhistory{\epsilon}
\def\effarrow#1{\stackrel{#1}{\rightarrow}}
\def\effpredarrow#1#2{\overset{\scriptscriptstyle #1}{\underset{\scriptscriptstyle #2}\rightarrow}}
\newcommand{\treeltfin}{\preccurlyeq_{\text{fin}}}
\newcommand{\treelt}{\preccurlyeq}
%\newcommand{\arrowht}[3]{#1\xrightarrow{#2} #3}
\newcommand{\nat}{\mathbb{N}}
\newcommand{\Trees}{\mathbb{T}}
\newcommand{\tree}{\varphi}
\newcommand{\treepath}{\pi}
\newcommand{\cut}[2]{#1\!\mid\!_{#2}}
\newcommand{\sig}{\varsigma}
\newcommand{\chk}{\phi}
\newcommand{\cardinal}[1]{|#1|}
\newcommand{\strace}{\varsigma}
\newcommand{\sctx}{\mathrm{sctx}}
\newcommand{\sctxs}{\mathrm{sctxs}}
\newcommand{\scod}[1]{\llparenthesis\,#1\,\rrparenthesis}
\newcommand{\cdummy}{c_{\mathrm{dummy}}}
\newcommand{\historify}[1]{\lfloor#1\rfloor}

\def\Subn{\Phi}
\def\merge{\mathit{M}}
\def\smerge{\mathit{M}_\subn}
\def\hmerge{\mathit{M}_H}
\def\tmerge{\mathit{M}_\tau}
\def\gmerge{\mathit{M}_\Gamma}
\def\humerge{\mathit{merge}_H^0}
\def\rmnabla{\not{\!\nabla}}
\def\mudnf{\mu\mathit{dnf}}
\def\zeight{\mathit{Z\mbox -8}}

\newcommand{\ctype}[2]{#1/#2}
\newcommand{\strip}[1]{\lfloor#1\rfloor}
\newcommand{\htobpa}[1]{\text{BPA}(#1)}
\newcommand{\Cset}[1]{\mathit{set}(#1)}
\newcommand{\clashes}{\asymp}

%% NEW HOOKADVICE MACROS BELOW
\long\def\cnote#1{{\small\textbf{\textit{\color{brown}(*#1 -- Chris*)}}}}%% NEW HOOKADVICE MACROS BELOW
\long\def\dnote#1{{\small\textbf{\textit{\color{blue}(*#1 -- David*)}}}}%% NEW HOOKADVICE MACROS BELOW
\long\def\tnote#1{{\small\textbf{\textit{\color{violet}(*#1 -- Tim*)}}}}
\long\def\jnote#1{{\small\textbf{\textit{\color{brown}(*#1 -- Joe*)}}}}
\long\def\xl#1{{\small\textbf{\textit{\color{blue}(*#1 -- Christelle*)}}}}
%\long\def\cnote#1{\marginpar{CS}{\small \ \ $\langle\langle\langle$\
%{#1 - CS}\
%    $\rangle\rangle\rangle$\ \ }} 
\newcommand{\openchan}{\fpkeyword{open}}
\newcommand{\chanread}[1]{#1.\fpkeyword{read}}
\newcommand{\chansubj}[1]{#1.\fpkeyword{subject}}
\newcommand{\chanwrite}[2]{#1.\fpkeyword{write}(#2)}
\newcommand{\subj}{\texttt{s}}
\newcommand{\subjs}{\bar{\subj}}
\newcommand{\subjvar}{\gamma}
\newcommand{\subjvars}{\bar{\alpha}}
\newcommand{\chan}{\mathbf{c}}
\newcommand{\exhm}[3]{\exists #1 . \{ #2, #3 \}}
\newcommand{\sett}[1]{\{ #1 \}}
\newcommand{\intt}{\mathit{int}}
\newcommand{\chant}[1]{\mathit{chan}[#1]}
%\newcommand{\chant}{\mathit{chan}}
\newcommand{\priv}{\pi}
%\newcommand{\hook}[2]{#1.\fpkeyword{auth}(#2)}
\newcommand{\hook}[1]{\fpkeyword{hook}(#1)}
\newcommand{\taintint}[1]{\intt_{#1}}
\newcommand{\taintv}[2]{{#1}\cdot{#2}}
\newcommand{\authev}[2]{#1\ \fpkeyword{requires}\ #2}
\newcommand{\authevq}[2]{#1\ \fpkeyword{requires}^?\ #2}
\newcommand{\indflowev}[2]{#1 \hookrightarrow #2}
\newcommand{\flowev}[2]{#1 \leadsto #2}
\newcommand{\flowevq}[2]{#1 \leadsto^? #2}
\newcommand{\deltaty}[4]{#1 \rightarrow \Delta #2 . #4,#3}
\newcommand{\fixty}[3]{#1 \rightarrow #2,#3}
\newcommand{\svec}{\bar{\subj}}
\newcommand{\freesubs}[1]{\mathrm{subjects}(#1)}
\newcommand{\subjt}{\varsigma}
\newcommand{\subjts}{\bar{\subjt}}
\newcommand{\tjudge}[5]{#2 \vdash_{#1} #4 : #5 \cdot #3}
\newcommand{\redx}{\rightarrow}
\newcommand{\redxs}{\redx^{*}}
\newcommand{\chanv}[1]{\langle #1 \rangle}
\newcommand{\acp}{\mathcal{A}}
\newcommand{\ifp}{\mathcal{F}}
\newcommand{\hooklang}{\Lambda_{\mathit{hook}}}
\newcommand{\rv}{\mathit{rv}}
\newcommand{\ksubject}{\textit{Subj}}
\newcommand{\kpc}{\textit{PC}}
\newcommand{\pow}[1]{\mathit{pow}(#1)}


\newcommand{\store}{\Sigma}
\newcommand{\loc}{\ell}
\newcommand{\eref}[1]{\fpkeyword{ref}\ #1}
\newcommand{\reft}[1]{\fpkeyword{ref}\ #1}
\renewcommand{\initenv}{\mathcal{E}}
\renewcommand{\subn}{\varrho}
\newcommand{\readpriv}{\mathbf{r}}
\newcommand{\writepriv}{\mathbf{w}}
\newcommand{\closeacp}{\mathrm{close}}

\newcommand{\fvar}{\alpha}
\newcommand{\flab}{\ell}
\newcommand{\fty}{\phi}
\newcommand{\flabty}[2]{#1^{#2}}
\newcommand{\recty}[1]{\{ #1 \}}
\newcommand{\labof}{\mathit{lab}}
\newcommand{\lattice}{\mathcal{L}}
\newcommand{\latel}{p}
\newcommand{\hilab}{\fpkeyword{hi}}
\newcommand{\lolab}{\fpkeyword{lo}}
\newcommand{\flowmap}{\mathcal{K}}
\newcommand{\subjlevels}{\flowmap_{\mathit{pol}}}
\newcommand{\ilab}{\subj}
\newcommand{\sle}{\preccurlyeq}
%\newcommand{\declass}[2]{\lfloor#2\rfloor_{#1}}
\newcommand{\declass}[2]{#2\!\downarrow_{#1}}
\newcommand{\halfmeet}[2]{#1\,\sqcap_{#2}}
\newcommand{\readf}{\mathrm{read}}
\newcommand{\writef}{\mathrm{write}}
\newcommand{\oklab}{\mathrm{ok}}
\newcommand{\badlab}{\mathrm{bad}}
\newcommand{\assignev}[2]{#1 \leftarrow #2}
\newcommand{\shookev}[1]{\mathit{check}(#1)}
\newcommand{\tr}{\theta}
\newcommand{\stepone}{\mathit{step}}
\newcommand{\steptwo}{\bar{\stepone}}
\newcommand{\stepthree}{\hat{\stepone}}
%\newcommand{\traceinterp}[1]{\llbracket #1 \rrbracket}
\newcommand{\hooktruncate}[1]{\lfloor #1 \rfloor}
\newcommand{\acl}{\mathcal{A}}
\newcommand{\mi}[1]{\mathit{#1}}
\newcommand{\ttt}[1]{\ensuremath{\mathtt{#1}}}

\newcommand{\ourprot}{\ensuremath{\mathrm{SHARD}}\xspace}


==> conclusion.tex <==
\section{Conclusion}\label{sec:con}

We propose a new highly scalable secure aggregation protocol, \emph{\ourprot}, with much better performance in cases with small vectors or many dropped out parties. 
\ourprot scales gracefully to accommodate hundreds of millions of parties while requiring only hundreds of connections per party in the vast majority of settings. 
Considering a malicious adversary requires changing very little about the protocol run, and does not substantially affect communication or computation costs. We simply require one additional share per group, and perform the reconstruction twice. 
Our empirical results show that \ourprot can aggregate over very large federations with a very small computational cost.

A small vector secure aggregation protocols have applications in distributed data analytics as well as smaller machine learning models. Histograms, random forests, logistic regression, and small neural networks would all benefit from protocols enabling short vector aggregation~\cite{fedforests,fedlog}


We leave for future work a further exploration of sharding configurations in secret sharing.
Our experiments have led us to believe that $2$ shards per party is optimal for this protocol,
however tighter approximations of the probability of a security failure could imply that more rounds of sharding are indeed optimal. 
Furthermore, more rounds of sharding open the possibility of packed secret sharing within the sharding round, and a protocol that better supports wider vectors.

